Verifying Classification with Limited Disclosure

We consider the multi-party classification problem introduced by Dong, Hartline, and Vijayaraghavan (2022) motivated by electronic discovery. In this problem, our goal is to design a protocol that guarantees the requesting party receives nearly all responsive documents while minimizing the disclosure of nonresponsive documents. We develop verification protocols that certify the correctness of a classifier by disclosing a few nonresponsive documents. We introduce a combinatorial notion called the Leave-One-Out dimension of a family of classifiers and show that the number of nonresponsive documents disclosed by our protocol is at most this dimension in the realizable setting, where a perfect classifier exists in this family. For linear classifiers with a margin, we characterize the trade-off between the margin and the number of nonresponsive documents that must be disclosed for verification. Specifically, we establish a trichotomy in this requirement: for $d$ dimensional instances, when the margin exceeds $1/3$, verification can be achieved by revealing only $O(1)$ nonresponsive documents; when the margin is exactly $1/3$, in the worst case, at least $\Omega(d)$ nonresponsive documents must be disclosed; when the margin is smaller than $1/3$, verification requires $\Omega(e^d)$ nonresponsive documents. We believe this result is of independent interest with applications to coding theory and combinatorial geometry. We further extend our protocols to the nonrealizable setting defining an analogous combinatorial quantity robust Leave-One-Out dimension, and to scenarios where the protocol is tolerant to misclassification errors by Alice.

==> Algorithm/Algo_Robust_Protocol.tex <==
\begin{algorithm2e}[htb]
\caption{Robust Critical Points Protocol}
\label{alg:robust_protocol}
\DontPrintSemicolon
\LinesNumbered

\KwIn{Subroutine for computing robust critical points (\Cref{alg:robust_critical}), Labeled points from Alice}
\KwOut{A subset of points sent to Bob}

Alice sends all points $X$ to Trent\;
Alice reports to Trent a set $X_A^+ \subseteq X$ as positive ($X_A^- = X \setminus X_A^+$ as negative)\;

% \If{Alice's report $(X_A^+, X_A^-)$ is not separable by a $\gamma$-margin linear classifier}{
%     Trent sends all points $X$ to Bob and the protocol ends\;
% }

Trent computes the critical points $C(X_A^+)$ using Algorithm~\ref{alg:robust_critical} with input $X_A^+$\;
Trent sends points $X_A^+ \cup C(X_A^+)$ to Bob\;
Bob labels the points and sends labels to Trent\;
Trent checks the agreement of reports from Alice and Bob and sends any disputed points to the court to settle\;

\If{the court disagrees with Alice's label on any disputed points}{
    Trent sends all points $X$ to Bob\;
}

\end{algorithm2e}


==> Paper/hard_instance.tex <==
%\subsection{Hard Small Margin Instances}\label{sec:hard}

\begin{lemma}[Constructing Skew-Obtuse Family of Vectors when margin $\gamma\leq 1/3$]
\label{lemma:constructing_skob_family}
    For any $\gamma \leq 1/3$, there exists an instance that can be separated by a linear classifier with margin $\gamma$ such that all negatives must be revealed to achieve recall $1$. 
\end{lemma}

The proof of Lemma~\ref{lemma:constructing_skob_family} is in Appendix~\ref{apx:constructing_skob_family}.

% \begin{proof}
%      Let $\varepsilon = 1/\sqrt{3}$.
%     We first consider the case when $\gamma =1/3$.
%    The dataset $X$ contains $n$ data points $x_1,\dots,x_n$ in $\bbR^{n+1}$ such that 
%     $$
%     x_i = \varepsilon \cdot e_1 + \sqrt{1-\varepsilon^2} \cdot e_{i+1},
%     $$
%     where $e_i$ is the $i$-th standard basis vector. Each data point $x_i$ has a unit length. 

%     Consider the following $n$ different label functions $f_1,\dots, f_n$ on this dataset $X$. The function $f_i$ labels the point $x_i$ as positive and all other points as negative. 
%     Let $h_i$ be the linear classifier with the weight vector $w_i = -\varepsilon \cdot e_1 + \sqrt{1-\varepsilon^2} \cdot e_{i+1}$. Then, we have $\inner{h_i}{x_i} = 1-2\varepsilon^2  \geq \gamma$ and $\inner{h_i}{x_j} = -\varepsilon^2  \leq -\gamma$ for all $j \neq i$. 
%     Thus, each instance $(X,f_i)$ is linear separable by margin $\gamma$ and $h_i$ is a $\gamma$-margin classifier for this instance $(X,f_i)$. Therefore, to distinguish these instances and achieve recall $1$, any protocol must reveal all data points for verification.

%     Next we consider the case when $\gamma = 1/3 - \eta$ for some $\eta >0$.
%     Let $\beta = (3/2)\eta$.
%     It is well-known that by picking unit vectors randomly in $\R^d$ we can construct a collection of vectors $v_1, v_2, \ldots v_k$ such that $\inner{v_i}{v_j} \leq \beta$ if $i\neq j$ and $k\geq \exp{(\Omega(\beta^2 d))}$ (see \Cref{lem:exp_many_neearly_orthogoanl_vectors} in the appendix for a proof). 
%     WLOG we can assume that $v_1,\ldots,v_k$ are in the span of $e_2,\ldots,e_{d+1}$. Now, for all $i\in [k]$ we set 
%     $$
%     x_i = \varepsilon \cdot e_1 + \sqrt{1-\varepsilon^2} \cdot v_{i}.
%     $$
%     Further, by setting $w_i = -\varepsilon \cdot e_1 + \sqrt{1-\varepsilon^2} \cdot v_i$ we have that 
%     \[
%     \inner{v_i}{w_i} = -\varepsilon^2 + 1 - \varepsilon^2 = 1/3 \geq \gamma
%     \]
%     and for $i\neq j$
%     \[
%     \inner{v_i}{w_j} \leq -\varepsilon^2 + (1 - \varepsilon^2)\eta = -1/3 + \eta = -\gamma.
%     \]
% \end{proof}

==> Paper/large_margin_protocol.tex <==
\subsection{Linear Classification with Margin}

In this section, we provide an E-Discovery protocol for realizable instances with large margins. 

\begin{theorem}\label{thm:protocol_realizable}
    For any instance linearly separable by margin $\gamma > 1/3$, there is a protocol that takes $\gamma$ as input and satisfies
    \begin{enumerate}
        \item (Recall) The recall is $1$.
        \item (Non-responsive disclosure) If Alice reports all labels truthfully, the non-responsive disclosure is at most 
        $$
        \frac{2+2\gamma}{3\gamma -1}.
        $$
        \item (Truthful) Alice's best strategy is to truthfully report all labels. 
    \end{enumerate}
\end{theorem}

\input{Algorithm/Algo_Protocol}
\input{Algorithm/Algo_Critical}

\begin{proof}[Proof of Theorem~\ref{thm:protocol_realizable}]
    The protocol first asks Alice to report labels of all documents in $X$ to Trent. Then, Trent checks whether the labels reported by Alice are linear separable by a $\gamma$-margin classifier. If the labels reported by Alice are not linear separable by margin $\gamma$, then reveal all documents to Bob. 
    
    Now suppose the labels reported by Alice are linear separable by margin $\gamma$. Let $X_A^+$ and $X_A^-$ be the set of all positives and the set of all negatives reported by Alice, respectively. Then, let $\calH_\gamma$ be the set of all linear classifiers that satisfy the following conditions: (1) all points in $X_A^+$ are still classified as positive; and (2) the margin of the classifier is at least $\gamma$; and (3) at least one point in $X_A^-$ is classified as positive. 
    
    We first show that $C_\gamma(X_A^+)$ can distinguish two cases: (1) the labels reported by Alice are correct; and (2) Alice labels some true positive points as negative, i.e. the true classifier is in $\calH_\gamma$. 
    Specifically, we show that for any classifier $h \in \calH_\gamma$, there exists a critical point in $C_\gamma(X_A^+)$ classified as positive by $h$. 
    Note that critical points $C_\gamma(X_A^+) \subseteq X_A^-$. 
    If all critical points $C_\gamma(X_A^+)$ are true negative, then we have case (1); otherwise, we are in case (2).
    We show this by contradiction. Suppose there is no point in $C_\gamma(X_A^+)$ classified as positive by $h$. 
    Consider any classifier $h \in \calH_\gamma$ that classifies at least a point in $X_A^-$ as positive. We use $X_h^+ = \{x \in X: h(x) = 1\}$ to denote the points classified as positive by $h$. Then, we have $X_h^+ \cap X_A^- \neq \varnothing$. Since no point in $C_\gamma(X_A^+)$ is classified as positive by $h$, all points in $X_h^+ \cap X_A^-$ are removed in Algorithm~\ref{alg:large_margin_critical}. Now, consider the last point $x_i$ in $X_h^+ \cap X_A^-$ that are removed in Algorithm~\ref{alg:large_margin_critical}. Let $M_i$ be the set $M$ at the beginning of the iteration at point $x_i$. Since $x_i$ is the last point in $X_h^+ \cap X_A^-$, we have $M_i \setminus \{x_i\} \cap X_h^+ = \varnothing$. Thus, $T_1 = X_A^+ \cup \{x_i\}$ and $T_2 = M_i \setminus \{x_i\}$ are separated by a $\gamma$-margin linear classifier $h$, which implies that $x_i$ is not removed. 

    Suppose $C_\gamma(X_A^+)$ contains $k$ points $v_1,v_2, \dots, v_k \in X$. We now show that for each $v_i$, there exists a linear classifier $h_i$ satisfies two properties: (1) $h_i(v_i) = 1$ and $h_i(v_j) = -1$ for all $j \neq i$; and (2) $h_i$ has a margin $\gamma$ on $C_\gamma(X_A^+)$. ($h_i$ is not required to be in $\calH_\gamma$.) Consider the iteration corresponding to the point $v_i$ in Algorithm~\ref{alg:large_margin_critical}. Let $M_i$ be the set $M$ at the beginning of this iteration. Since $v_i$ is not removed, there is a $\gamma$-margin linear classifier $h$ that separates $\{v_i\}$ from $M_i \setminus \{v_i\}$. Note that the critical points $C_\gamma(X_A^+)$ is a subset of $M_i$. This classifier $h$ satisfies two properties for the point $v_i$.
    
    % Let $S \subseteq X_A^-$ be the smallest set that satisfies for any classifier $h \in \calH_\gamma$, if $h$ classifies any point in $X_A^-$ as positive, then there exists a point in $S$ classified as positive by $h$. Suppose $S$ contains $k$ points $v_1,v_2, \dots, v_k \in \bbR^d$. For each $v_i$, there exists a classifier $h_i \in \calH_\gamma$ such that $h_i(v_i) = 1$ and $h_i(v_j) = -1$ for all $j \neq i$. If there is no such $h_i$, then we can remove $v_i$ from $S$ and get a smaller set satisfying the condition. 
    
    Let $w_i \in \bbR^d$ be the unit-length weight vector of the classifier $h_i(x) = \sgn(\inner{w_i}{x})$. Let $\bar{v}_i = v_i/\|v_i\|_2$. Since $h_i$ has margin at least $\gamma$, we have $\inner{\bar{v}_i}{w_i} \geq \gamma$ and $\inner{\bar{v}_j}{w_i} \leq -\gamma$ for any $j \neq i$. 

    
    Therefore by Lemma~\ref{lemma:skew-obtuse_lemma}, we have the number of points in $C_\gamma(X_A^+)$ is at most 
    $$
    k \leq \frac{2+2\gamma}{3\gamma-1}.
    $$
\end{proof}



==> header/notations.tex <==
%% probability notation
\DeclareMathOperator{\cov}{cov}
\DeclareMathOperator{\sgn}{\mathbf{sgn}}
\DeclareMathOperator{\E}{\mathbf{E}}
\DeclareMathOperator{\Var}{\mathbf{Var}}
\DeclareMathOperator{\one}{\mathbf{1}}
\newcommand{\given}{\mid}
\DeclareMathOperator{\Ball}{Ball}
\DeclareMathOperator{\tr}{tr}

% rounding up and down
\newcommand {\roundup}   [1] {{\lceil {#1} \rceil}}
\newcommand {\rounddown} [1] {{\lfloor {#1} \rfloor}}

%% black board letters
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbZ}{\mathbb{Z}}

%% calligraphic letters 
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}

\newcommand{\N}{\mathbb{N}}
\newcommand{\R}{\mathbb{R}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}




\newcommand{\err}{\mathrm{err}}
\newcommand{\errstar}{\mathrm{err}^*}

\DeclareMathOperator{\REC}{REC}
\DeclareMathOperator{\NRD}{NRD}
\DeclareMathOperator{\FN}{FN}
\DeclareMathOperator{\FP}{FP}

\DeclareMathOperator{\Tr}{Tr}

\newcommand{\conv}{\mathrm{conv}}
\newcommand{\cone}{\mathrm{cone}}
\newcommand{\inner}[2]{\langle #1, #2\rangle}
% \newcommand{\sid}[1]{\textcolor{cyan}{#1}}
% \newcommand{\todosid}[1]{\textcolor{red}{#1}}
